Mono3R: Exploiting Monocular Cues for Geometric 3D Reconstruction

Recent advances in data-driven geometric multi-view 3D reconstruction foundation models (e.g., DUSt3R) have shown remarkable performance across various 3D vision tasks, facilitated by the release of large-scale, high-quality 3D datasets. However, as we observed, constrained by their matching-based principles, the reconstruction quality of existing models suffers significant degradation in challenging regions with limited matching cues, particularly in weakly textured areas and low-light conditions. To mitigate these limitations, we propose to harness the inherent robustness of monocular geometry estimation to compensate for the inherent shortcomings of matching-based methods. Specifically, we introduce a monocular-guided refinement module that integrates monocular geometric priors into multi-view reconstruction frameworks. This integration substantially enhances the robustness of multi-view reconstruction systems, leading to high-quality feed-forward reconstructions. Comprehensive experiments across multiple benchmarks demonstrate that our method achieves substantial improvements in both mutli-view camera pose estimation and point cloud accuracy.

==> Figures/mono-pair-supply.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{Figures/mono-pair-supply_fig.pdf}
  \caption{
    Qualitative comparision of Mono3R and DUSt3R.
  }
  \label{fig:mono-pair-supply}
\end{figure}

==> Figures/quality-supply.tex <==
\begin{teaserfigure}
  \includegraphics[width=\textwidth]{Figures/quality-supply_fig.pdf}
  \caption{
    Qualitative comparision of Mono3R and DUSt3R.
}
  \label{fig:quality-suppl}
\end{teaserfigure}
